Multi-fidelity Stability for Graph Representation Learning

In the problem of structured prediction with graph representation learning (GRL for short), the hypothesis returned by the algorithm maps the set of features in the \emph{receptive field} of the targeted vertex to its label. To understand the learnability of those algorithms, we introduce a weaker form of uniform stability termed \emph{multi-fidelity stability} and give learning guarantees for weakly dependent graphs. We testify that ~\citet{london2016stability}'s claim on the generalization of a single sample holds for GRL when the receptive field is sparse. In addition, we study the stability induced bound for two popular algorithms: \textbf{(1)} Stochastic gradient descent under convex and non-convex landscape. In this example, we provide non-asymptotic bounds that highly depend on the sparsity of the receptive field constructed by the algorithm. \textbf{(2)} The constrained regression problem on a 1-layer linear equivariant GNN. In this example, we present lower bounds for the discrepancy between the two types of stability, which justified the multi-fidelity design.

==> sections/6.tex <==
% Pruning is a natural method to greedily approximate solutions of problem \ref{op}. One common assumption for the graph that existed naturally is that it is sampled from a scale-free infinite network~\citep{stumpf2005subnets}, which follows the power-law degree distribution. Some previous attempts have been made to find better solutions of graph sampling in terms of the structural similarity to the original one.~\citep{leskovec2006sampling}. The key intuition borrowed from these works is that all sampling methods will somehow damage the degree distribution of the original graph. Pruning in random can also be seen as a type of edge sampling that will shift the distribution of the original graph, causing information damage on the graph. Therefore the typical problem would be: \textit{How to find a good strategy to handle the distribution shift ?}
The results presented in the previous sections suggest that sparsity of receptive field plays a key role in the stability-based learning guarantees. 

In this section, we obtain guarantees for sparsity regularization method. Contrary to the sparsity regularization in LASSO~\citep{tibshirani1996regression} on sparse regression and compressed sensing, the problem considered here only concerns the size of the receptive field, a key structural property. Our proposition of this method is to argue for a better guarantee by leveraging the trade-off between bias and variance. This is often referred to as structural risk minimization by ~\citet{vapnik1999overview}. The estimator we construct by sparsity regularization is
\begin{align*}
\label{h}
    h^{\tt{sparse}}&=\argmin_{h\in\ca H_d}\wh R(h)\\
    \text{ Or, }h^{\tt{sparse}}&=\argmin_{h\in\ca H}\wh R(h)+2\lambda d(h)\beta_2&\tag{*}
\end{align*}
{\color{red}  these two options are different right? which one of the two are you using? Use the simpler one}
with $d(h)\in[1,\dmax]$ is the truncated maximum degree s.t. $d(h)=\inf\{d:h\in\ca H_d\}$ and $\ca H_d\subseteq \ca H$ is the sub-hypothesis set with maximum degree $d$ and $\lambda>0$ is the scaled slack variable. We have the following guarantee for it:
\begin{theorem}[Learning Guarantee of Sparse GRL]
Suppose $\ca H=\bigcup_{d=1}^{d_{\max} }\ca H_d$ is the union of the class of graph representation learning models with sparsity $d$, let $h^{\mathtt{sparse}}$ be the algorithm returned by \ref{h}, and $\epsilon\geq \sup_d 2(2-\lambda)d\beta_2$ then the following holds with probability at least $1-2\sum_{d=1}^\dmax \exp\left(\frac{-(\epsilon/2+(\lambda-2)d\beta_2)^2}{2N((2-2d)\beta_1+d(\beta_2+B_{L}))^2}\right)$:
\begin{equation*}
   R(\hsp)\leq\inf_{h\in\ca H}\left(R(h)+(\lambda+2)d(h)\beta_2\right)+\epsilon
\end{equation*}
\end{theorem}
\begin{remark}
Note that as $\lambda$ scales up, the first term on R.H.S. will significantly increase while the second one will decrease under some fixed confidence interval. This creates a trade-off between the estimation and approximation error using the parameter $\lambda$.
% It is easy to see that $\lambda$ governs the tradeoff between the approximation error and the estimation error of the model. However, we will need to perform $O(d)$ times of iteration to find the optimal sparsity. This can be computationally expensive when $d$ is very large, which stays as a major limitations for this problem. Random algorithm like DropEdge~\citep{Rong2020DropEdge} was proposed and exemplifies the idea of sparse regularization.
\end{remark}
{\color{red} 
This section needs more work: it is not sufficiently grounded in the related works that also consider sparse regression. Also, the connection with the other sections is not fleshed out sufficiently. How does Theorem 10 relate to the other theorems? 
Also, if you denote by $\delta = 2\sum_{d=1}^\dmax \exp\left(\frac{-(\epsilon/2+(\lambda-2)d\beta_2)^2}{2N((2-2d)\beta_1+d(\beta_2+B_{L}))^2}\right)$, explain the nature of this bound. What are the important parameters to look for here? 
}

% Sparsity regularization has been extensively used in linear classifiers like margin-based SVMs. However, the sparsity here is not related to data sparsity, but edge sparsity in the graph. Sparsity regularization reduced the expected degree on the graph to a large degree. Empirical work like DropEdge ~\citep{Rong2020DropEdge} has demonstrated that random dropout on edge might lead to better performance on graph neural networks. However, their heuristic based work is based on empirical evidence and their strategy is only applicable to GNNs. The sparsity regularization we performed, however, is generalizable to any graph representation learning frameworks. Our simulation results suggested that the regularization strategy can improved the model performance on inductive learning tasks even if the graph that we used for training and testing are different in structure but share some implicit similarities. Hence, sparse graph model is remarkable that it is not only guaranteed with generalization bound, but also works well in practice.
% \begin{compactenum}
%  \item It can maximally keep the original computational graph structure while effectively reducing the global maximum degree. We measure this property through the Maximum Degree Ratio (MDR for short). MDR is the ratio of the branching factor of the pruned graph to the original graph, being a monotonically decreasing value with the pruning ratio.
% \item Remain relatively close to the overall global of the graph before pruning. We measure this through the symmetric Jensen-Shannon Divergence of the degree distribution between the pruned graph and the original one (JSD for short) because the distribution is closely related to the stability-induced generalization bound.
% \end{compactenum}

% In the following subsections, we detailed the SR-GNN frameworks and made extensive comparisons between some varieties of it.
% \begin{algorithm}[htbp]
%   \caption{Training SR-GNN with Bagging and SGD}
%       \label{alg:naive}
%     \begin{algorithmic}[1]
%     \REQUIRE Graph $\mathcal{G}$, GNN $f_\theta$
%     \REQUIRE Rate $\{\psi_i\}_{i\in [M]}$
%   \STATE Randomly initialize $\theta$
% %   \STATE Compute maximum degree of $\mathcal{G}$ as $d$
%       \FOR{$i=0$ {\bfseries to} $M$}
%       \IF{Pruning before bagging}
%           \STATE $\ca G = \mathtt{prune}(\ca G, \psi)$
%         \ENDIF
%           \STATE Randomly sample batches of subgraphs $\{g_i\}$ 
%           \FOR{$j=0$ {\bfseries to} $N$}
%               \FOR{{\bfseries all $g \in \{g_i\}$ }}
%                     \STATE Construct Conputation Tree Set \\
%                     $\ca S = \{\ca T_1,..., \ca T_{|g_i|}\}$
%                   \IF{Bagging before pruning}
%                     \STATE $g = \mathtt{prune}(g, \psi_i)$
%                     \ENDIF
%                     \STATE Calculate gradient $\nabla_\theta \mathcal{L}_{g}(f_\theta,\ca S)$
%                     \STATE Update parameters with gradient:\\ 
%                     $\theta = \theta - \alpha \nabla_\theta\mathcal{L}_{g}(f_\theta,\ca S)$
%                 \ENDFOR
%             \STATE Evaluate $f_\theta$
%             \ENDFOR
%       \ENDFOR
%   \vskip -0.9in
% \end{algorithmic}
% \end{algorithm}
% \subsection{Pruning with Random Edge Selection} 
% To use random edge selection as the pruning strategy, $(1-\psi) |E|$ edges are dropped from the graph randomly. With the same pruning rate (e.g. the rate of left edges count versus the total count), simulation results imply that graphs pruned with this method is closer to the degree distribution of the original graph with lower JSD, indicating better structural similarities. However, it suffered from high MDR, indicating that we will be removing a lot of local details from the graph to scale down the branching factor. A similar method, DropEdge, was proposed in ~\citet{Rong2020DropEdge}. DropEdge, as its name suggests, drops edges according to the Bernoulli distribution. However, DropEdge is not an efficient method in approximating SR-GNN since we can neither control the branching factor $d$ nor the size of the sample. 

% Then we briefly analyze how pruning affects the generalization of SGD-trained GNNs with the uniformly randomized pruning operator.

% \begin{definition}
% A random map $D: \Omega\rightarrow \Omega$ is a pruning operator with rate $s$ if for every computation tree $\ca T\in\Omega$ we have $\bb E\Vert f(D\ca T)\Vert = s\Vert f(\ca T)\Vert$. Then for the differentiable function $f: \Omega\rightarrow\Omega$, using $DG_{f,\alpha}$ to denote the gradient update with pruning that is formalized as $DG_{f,\alpha}(\ca T_v) = v- \alpha \nabla f(D\ca T_v)$ on node $v$ and its computation tree $\ca T_v$ 
% \end{definition}

% Theorem \ref{thm:bound} would be modified in 2 parts with the introduction of random pruning:
% \begin{compactenum}
%  \item The term related to the statistics of edge
%  \item The Lipschitz constant $L$
% \end{compactenum}
% The first one is straight-forward. We briefly discuss the effect of pruning operator on the constant $L$ in the bound:

% \begin{lemma}
% \label{lm: liptz}
% Assume that $f$ is L-Lipschitz. Then, $DG_{f,\alpha}$ with pruning rate $s$ is ($s\alpha L$)-bounded.
% \end{lemma}
% We delay the proof to the appendix.
% The lemma \ref{lm: liptz} indicates that we can replace $L$ with $sL$ in the theorem. Therefore, random pruning, besides being efficient in scaling down the generalization bound directly as \textit{Weight Decay}, has a similar effect of stochastic regularization as \textit{Dropout}.

% % Iterative pruning has been a popular technique in Neural Network Pruning studied by ~\citet{han2015learning} to compress the model, which was extensively studied in ~\citet{frankle2018lottery}.  We get insights from their approach and applied this technique to our graph pruning. Iterative pruning provides better initialization and shortens the total time to converge in the context of network pruning.
% \subsection{Pruning with Truncation}
% Another direction would be to randomly truncate the graph. (e.g. pick nodes with a high degree and prune the randomly-selected edges connecting to them.) Truncation is a very efficient way of scaling down the branching factor while maintaining almost all of the low-degree details in the graph, which makes it a strong method in the local view. However, this method is highly biased to the nodes with high degrees.

% The above analysis implies that both methods bear advantages and limitations. Then a straightforward strategy is using a hybrid approach where the two algorithms are combined sequentially, with $\lambda sE$ and $(1-\lambda)sE$ being pruned respectively with the two methods. We did experiments on this simple hybrid method with $\lambda = \frac{1}{2}$ in the next section.
% \begin{align*}
% \end{align*}
% % Algorithm \ref{alg:naive} is the naive version of iterate pruning in training GNNs. The rationale of this algorithm lies in the generalization bound we obtained in \ref{sect:three} as we have a better generalization bound when the maximum degree $d$ is bounded. However, the major drawback behind it is also crucial: we compromised the original dataset. Pruning deviates the original sample distribution $\mathcal{D}$ into $\hat{\mathcal{D}}$, which is causing the distribution we learned to be different from the original one. This lifted the generalization error. However, the two factors are resisting each other during pruning. In our empirical evaluation, this tradeoff can be utilized to lift the performance of GNNs on multiple datasets detailed in \ref{sect:five}. 
% \begin{figure}
% \begin{tabular}{rc}
% %     \multicolumn{2}{l}{\includegraphics[width=.45\textwidth]{figures/fig_toget.png}}\\
% % \quad\quad\quad(a) Random&(b) Truncation\\
%      \multicolumn{2}{l}{\includegraphics[width=.48\textwidth]{figures/together_plot-01.jpg}}\\
% \quad\quad\qquad(c) JSD &(d) MDR\\
% \end{tabular}
% % \caption{\textbf{Top:} Degree distribution of graph (on the Cora graph dataset) pruned at different percentage. We did kernel density estimation and plot the vertices with degree less than 25. The density corresponds to the left number of edges vs the total number of edges. \textbf{Bottom:} JSD and MDR value for two algorithms, where x-axis represents the proportion of left edges in the graph and y-axis represents the corresponding metric value we used to evaluate the random pruning algorithms }
% \caption{JSD and MDR value for two algorithms, where x-axis represents the proportion of left edges in the graph and y-axis represents the corresponding metric value we used to evaluate the random pruning algorithms }
% \label{prune}
% \end{figure}

% \subsection{Bagging Scenarios}
% When the graph is so large that we need to form mini-batches to adapt to the computation limits, bagging algorithm is used as a surrogate to the full graph learning. It runs on $T$ different subsets of training set $\ca D$ and averages the obtained solutions. We denote the subset by $\ca D(\bfa r_t)$ for $t=1,...,T$ where $\bfa r_t\in \ca R=\{1,...,m\}^m$ are instances of random variable corresponding to sampling with replacement of $m$ elements that forms the training set $\ca D$. Such random variables have multinomial distribution with parameters $\big(\frac{1}{m},...,\frac{1}{m}\big)$. The model can be written as 
% \begin{equation*}
%     F_{\ca D, \bfa r}= \frac{1}{T}\sum_{t=1}^{T}f_{\ca D(\bfa r_t)}
% \end{equation*}
% with the assumption that the base learning method $f_{\ca D}$ treats multiple copies of a training point as one point. We can incorporate the bagging scenario into the random stability framework~\citep{elisseeff2005stability}, where:
% \begin{theorem}[Random Pointwise Stability]
% A randomized algorithm A has random pointwise hypothesis stability $\gamma_m$ w.r.t. the loss function $l$ if the following holds:
% \begin{equation*}
%     \forall i\in\{1,...,m\}, E_{\ca D, \bfa r, z}[|l(f_{\ca D, \bfa r, z})-l(f_{\ca D^{\setminus i} \cup z, \bfa r,z })|]\leq \gamma_m
% \end{equation*}
% \end{theorem}
% \begin{lemma}
% \label{lm:8}
% Assume that the loss $l$ is $B$-Lipschitz w.r.t its first variable. Let $F_{\ca D, \bf r}$,where $ \mathbf{r}\in \ca R^T$, be the outcome of a bagging algorithm whose base machine has point-wise hypothesis stability $\beta_m$ w.r.t. the $l_1$ loss function. Then the random hypothesis stability $\gamma_m$ of $F_{\ca D, \bf r}$ w.r.t. $l$ is bounded by 
% \begin{equation*}
%     \gamma_m\leq B\sum_{k=1}^{m}\frac{k\beta_k}{m}\bb P_{\bfa r}[d(\bfa r)=k]
% \end{equation*}
% where $d(\bfa r),\in \ca R$, is the umber of distinct sampled points in one iteration.
% \end{lemma}
% And the corresponding performance bound is also guaranteed as:
% \begin{theorem}[Random Pointwise Stability Bound]
% \label{thm: bag}
% Let $f_{\ca D \bfa r}$ be the outcome of a random algorithm with random pointwise hypothesis stability $\gamma_m$ w.r.t. a loss function $l$ s.t. $0\leq l(f,z)\leq M$, for all $y\in\ca Y,r\in \ca R$ and all set $\ca D$. Then with probability $1-\delta$ w.r.t. the random draw of $\ca D$ and $\bfa r$,
% \begin{equation*}
%     R(f_{\ca D, \bfa r})\leq \h R(f_{\ca D, \bfa r}) +\sqrt{\frac{2M^2 +12Mm\gamma_m}{m\delta}}
% \end{equation*}
% \end{theorem}
% As the $\beta_m$ term has already been established in the previous section, we can directly obtain the generalization guarantees for bagging scenario via theorem \ref{thm: bag}. Since $\beta_m$ is approximately $O(\frac{\bb E_m[d]}{m})$, assuming $d_{max}\ll m$, our random hypothesis stability bound for $\gamma_m$ would directly goes to $O(\frac{\bb E[d]}{m})$, scales linearly with the expectation of $d$.

% A natural question exists in the bagging scenario: \textit{Should we do bagging first or pruning first ?} The generalization study we performed in section \ref{sect:two} is optimization agnostic, only take into account the complexity measure of GNNs, indicating that pruning-before-bagging can improve generalization. The analysis of bagging algorithms and \ref{lm: liptz} guarantees the performance of the bagging-before-pruning scenario. Previous empirical work has also been focusing on the latter case ~\citep{Rong2020DropEdge}, which works empirically well on moderate-scale datasets. 


% \begin{algorithm}[tb]
%   \caption{Adaptive Pruning}
%   \label{alg:adaptive}
%     {\bfseries Require:} Original Graph $\mathcal{G}(V,E)$, Times of Pruning: $M$ \\
%     {\bfseries Require:} GNN $f_\theta$, Pruning Ratio $\psi$
%   \begin{algorithmic}[1]
%   \STATE Randomly initialize $\theta$
%       \FOR{$i=0$ {\bfseries to} $M$}
    
%           \STATE Randomly Sample batch of subgraphs $g_i \sim \mathcal{D}$ 
%           \STATE Initialize global loss buffer $\mathcal{L}$ as zero value
%           \WHILE{early stopping criteria {\bfseries not} satisfied}

%           \FOR{{\bfseries all $g_i$}}
%                 \STATE Evaluate $\nabla_\theta \mathcal{L}_{g_i}(f_\theta)$ with respect to K samples
%                 \STATE Update parameters with gradient descent:\\ 
%                 $\theta = \theta - \alpha \nabla_\theta\mathcal{L}_{g_i}(f_\theta)$
%                 \STATE Update $\mathcal{L}$ with $\mathcal{L}_{g_i}$
%             \ENDFOR
%             \STATE Evaluate $f_\theta$ on validation set
%             \ENDWHILE
%             \STATE Rank all the edges $(u,v)$ according to $|\mathcal{L}(u) - \mathcal{L}(v)|$
%             \STATE Prune the graph with respect to $\psi$ and drop $\psi |E|$ edges according to the rank
%       \ENDFOR
% \end{algorithmic}
% \end{algorithm}
% \vspace*{1cm}
